Fine-Tuning Large Neural Language Models for Biomedical Natural Language Processing

Motivation: A perennial challenge for biomedical researchers and clinical practitioners is to stay abreast with the rapid growth of publications and medical notes. Natural language processing (NLP) has emerged as a promising direction for taming information overload. In particular, large neural language models facilitate transfer learning by pretraining on unlabeled text, as exemplified by the successes of BERT models in various NLP applications. However, fine-tuning such models for an end task remains challenging, especially with small labeled datasets, which are common in biomedical NLP. Results: We conduct a systematic study on fine-tuning stability in biomedical NLP. We show that finetuning performance may be sensitive to pretraining settings, especially in low-resource domains. Large models have potential to attain better performance, but increasing model size also exacerbates finetuning instability. We thus conduct a comprehensive exploration of techniques for addressing fine-tuning instability. We show that these techniques can substantially improve fine-tuning performance for lowresource biomedical NLP applications. Specifically, freezing lower layers is helpful for standard BERT-BASE models, while layerwise decay is more effective for BERT-LARGE and ELECTRA models. For low-resource text similarity tasks such as BIOSSES, reinitializing the top layer is the optimal strategy. Overall, domainspecific vocabulary and pretraining facilitate more robust models for fine-tuning. Based on these findings, we establish new state of the art on a wide range of biomedical NLP applications. Availability and implementation: To facilitate progress in biomedical NLP, we release our state-of-the-art pretrained and fine-tuned models: https://aka.ms/BLURB.

==> old/old-discuss.tex <==
\section{Discussion}

A variety of neural language models have been proposed, including those based on recurrent neural networks \citep{elmo} and generative models


Recently, there has been increasing interest in applying pretrained neural language models to biomedical applications \citep{lee2020biobert,peng2019bluebert,mimicbert,pubmedbert}. However, focusing on pretraining


Recently \citet{10.1093/bioinformatics/btaa668} demonstrated how biomedical BERT models can be achieve state of the art performance on the classification of radiology text reports and event extraction \citep{10.1093/bioinformatics/btaa540}. Other approaches to mitigate the challenge of scarce data in the biomedical domain besides domain specific pre-training include multi-task learning \citep{10.1093/bioinformatics/btaa515}, however this is only possible for common tasks such as named-entity recognition.


In this paper, we explore how the process of training a biomedical language model can be simplified, by making appropriate adjustments to the pretraining and finetuning process.

Performance on the BLURB benchmark is highly sensitive to the performance of a model on sentence similarity and question answering tasks. These challenging tasks are comprised of few datapoints, reflecting the fact that it is difficult to obtain large labelled datasets in the biomedical domain for tasks that are more complex than named entity recognition and relation extraction. Larger language models, as illustrated by our PubMedBERT-Large can offer significant performance improvements on these challenging tasks, pushing the BLURB score to a new state of the art.

We also demonstrate how the next sentence prediction task can be dropped from the pretraining process with no loss in performance on the biomedical tasks in the BLURB benchmark..

We have similar observations as \citet{peters-etal-2019-tune} and so for the transformer models evaluated on BLURB we favour fine-tuning over feature extraction.

\eat{
\begin{table}[!ht]
\caption{Summary of techniques used to reduce the variance in model performance on the small datasets that are part of BLURB and are prone to fine-tuning}
\resizebox{.4791\textwidth}{!}{
\begin{tabular}{@{}ccccccc@{}}
    \hline
    & Domain
    & \multirow{2}{*}{\begin{tabular}{@{}l@{}}Freeze\\layers\end{tabular} } & \multirow{2}{*}{\begin{tabular}{@{}l@{}}Longer\\training\end{tabular} } & \multirow{2}{*}{\begin{tabular}{@{}l@{}}ADAM\\de-biasing\end{tabular} } & 
    \multirow{2}{*}{\begin{tabular}{@{}l@{}}Layer-wise\\decay\end{tabular} } & \multirow{2}{*}{\begin{tabular}{@{}l@{}}Layer\\reinit\end{tabular}}\\
    & & & & &\\
\midrule
\citet{griesshaber-etal-2020-fine} & General (GLUE) & \checkmark & & & & \\
\citet{mosbach2021on} & General (GLUE) & & \checkmark & \checkmark & & \\
\citet{zhang2021revisiting} & General (GLUE) & & \checkmark & \checkmark & & \checkmark \\
Ours & BioMed (BLURB) & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
\midrule
\botrule
\end{tabular}}{}
\label{table:stability_summary}
\end{table}
}

We employ four techniques listed in Table~7\vphantom{\ref{table:stability_summary}} when we evaluate models on the BLURB and they demonstrate fine-tuning instability. We choose to evaluate these four promising methods which are simple to implement, they require no additional or intermediate training and allow no selection of random seeds on test data. Other important methods include fine-tuning on intermediate tasks \citep{Phang2018SentenceEO}, which we avoid in this case due to the computational cost of this method, and  Mixout \citep{Lee2020Mixout:} which was not found it to consistently offer a better performance impact than the strategies employed by \citet{mosbach2021on} and \citet{zhang2021revisiting}. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%     please remove the " % " symbol from \centerline{\includegraphics{fig01.eps}}
%     as it may ignore the figures.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%% Error analysis into attention patterns
\eat{

Alternate fine-tuning strategies error analysis. On simple tasks like the NER task NCBI disease, the model is only required to contextualise tokens in a short sequence since entity names typically only consist of a small number of separate tokens. Figure~4\vphantom{\ref{fig:example1}} illustrates that for difficult entity names, which have challenging grammar, PubMedBERT fine-tuned with both alternate strategies struggles to contextualise all the tokens that make up the entity such as `and' and `the'.

\begin{figure}[!ht]
\centering
    \includegraphics[width=0.48\textwidth]{figs/attention_vis_ncbi.png}
    \caption{Comparing the final layer attention coefficients for PubMedBERT-Base on the NCBI disease NER task for the two cases where encoder layers are either frozen or removed.
    }
    \label{fig:example1}
\end{figure}

Removing layers causes the model to suffer a catastrophic collapse in performance on tasks such as the relation extraction task DDI. The model falls back to predicting the majority class (no relation) for nearly all the examples. We hypothesise that reducing the size of the encoder by so much for this tasks makes it impossible for the model to learn complex high-level linguistic features that are required to perform adequately. For example in Figure~5\vphantom{\ref{fig:example2}} the word `incompatible', which has the greatest attention for the model with encoder layers removed, is found in examples which have the label FALSE (no relation) over 90\% of the time in the training data. The model is required to contextualise `incompatible' with tokens such as `and' and `with' to recognise that this relation is in fact an interaction between two drugs.

\begin{figure}[!ht]
\centering
    \includegraphics[width=0.48\textwidth]{figs/attention_vis_ddi.png}
    \caption{Comparing the final layer attention coefficients for PubMedBERT-Base on the DDI relation extraction task for the two cases where encoder layers are either frozen or removed.
    }
    \label{fig:example2}
\end{figure}
}



==> old/old-method.tex <==
\begin{methods}
\section{Methods}

%{\bf HP: revise and simplify background materials}

% overview
In this paper, we focus our study on Bidirectional Encoder Representations from Transformers~(BERT)~\cite{devlin2018bert}, which has become a mainstay of neural language models in NLP applications. In this section, we review the core technical aspects in BERT pretraining and fine-tuning, and identify key research questions for our fine-tuning study.

% transformer / BERT: objective, vocab, optimization, layers
\subsection{Neural Language Models}
The input to a neural language model consists of text spans, such as sentences separated by special tokens~$\tt [SEP]$. To address the problem of out-of-vocabulary words, neural language models generate a vocabulary from subword units, using Byte-Pair Encoding~(BPE)~\cite{sennrich2015bpe} or variants such as WordPiece~\cite{kudo2018sentencepiece}.
Essentially, the BPE algorithm tries to greedily identify a small set of subwords that can compactly form all words in a given corpus. It does this by first shattering all words in the corpus and initializing the vocabulary with characters and delimiters.  It then iteratively augments the vocabulary with a new subword that is most frequent in the corpus and can be formed by concatenating two existing subwords, until the vocabulary reaches the pre-specified size (e.g., 30,000 in standard BERT models or 50,000 in RoBERTa~\cite{liu2019roberta}). In this paper, we use the WordPiece algorithm which is a BPE variant that uses likelihood based on the unigram language model rather than frequency in choosing which subwords to concatenate. 

The text corpus and vocabulary may preserve the case ($\tt cased$) or convert all characters to lower case ($\tt uncased$). Prior work such as \cite{gu2021domainspecific} finds that it doesn't have significant impact on downstream tasks, so by default we use the $\tt uncased$ version.

Bidirectional Encoder Representations from Transformers~(BERT)~\cite{devlin2018bert} is a state-of-the-art neural language model based on transformer \cite{vaswani2017attention}. 
The transformer model introduces a multi-layer, multi-head self-attention mechanism, which has demonstrated superiority in leveraging GPU computation and modeling long-range textual dependencies. 
Standard BERT pretraining inputs two text spans (e.g., sentences) and assigns a distinct segment ID to each. 
The input token sequence is first processed by a lexical encoder, which combines a token embedding, a position embedding and a segment embedding by element-wise summation. 
This embedding layer is then passed to multiple layers of transformer modules \cite{vaswani2017attention}. 
In each transformer layer, a contextual representation is generated for each token by summing a non-linear transformation of the representations of all tokens in the prior layer, weighted by the attentions computed using the given token's representation in the prior layer as the query.
The final layer outputs contextual representations for all tokens, which combine information from the whole text span.

BERT models come with two standard configurations: $\tt BASE$ uses 12 layers of transformer modules and 110 million parameters, $\tt LARGE$ uses 24 layers of transformer modules and 340 million parameters. Prior work in applying BERT to biomedical NLP tends to focus on $\tt BASE$ models. We consider $\tt LARGE$ models as well and study additional challenges in fine-tuning these larger models in biomedical NLP.

\subsection{Pretraining Objectives}
As in other language models, the key idea of BERT pretraining is to predict the held-out portion in unlabeled text. Unlike most prior language models, BERT does not adhere to a generative model. Instead, \citet{devlin2018bert} introduces two self-supervised objectives: \textbf{Masked Language Model} and \textbf{Next Sentence Prediction}. 
Masked language model (MLM) randomly replaces a subset of tokens by a special token (e.g., $\tt [MASK]$), and asks the language model to predict them. 
The training objective is the cross-entropy loss between the original tokens and the predicted ones. 
%In BERT and RoBERTa, 
Typically, 15\% of the input tokens are chosen, among which a random 80\% are replaced by $\tt [MASK]$, 10\% are left unchanged and 10\% are randomly replaced by a token from the vocabulary. % Instead of using a constant masking rate of 15\%, a standard approach is to gradually increase it from 5\% to 25\% with 5\% increment for every 20\% of training epochs, which makes pretraining more stable~\cite{liu2020alum}.  
Next sentence prediction (NSP) is a binary classification task that determines for a given sentence pair whether one sentence follows the other in the original text. 
While MLM is undoubtedly essential for BERT pretraining, the utility of NSP has been called into question in prior work~\cite{liu2019roberta}.
We will conduct simplified pretraining using MLM only and study how NSP and the use of segment IDs in pretraining might impact downstream fine-tuning performance. 

Besides from standard BERT pretraining objectives, we also consider ELECTRA \cite{clark-electra}, which has shown good performance in general-domain datasets such as GLUE~\cite{glue} and SQuAD~\cite{squad}. 
ELECTRA introduces an MLM-based generator to help pretrain a discriminator for use in end tasks. Specifically, given sample masked positions, first the generator predicts the most likely original tokens as in MLM, then the discriminator classifies for all tokens whether each is the original one.
While ELECTRA shares some superficial similarity with generative adversarial network (GAN)~\cite{gan}, the roles of generator and discriminator are very different. After pretraining, the generator in ELECTRA is discarded and the discriminator is used for downstream fine-tuning, which is the opposite of GAN. The training objective is not adversarial, but rather a weighted combination of MLM for the generator and classification accuracy for the discriminator. By classifying on all tokens rather than just the masked ones, ELECTRA can potentially learn more from each example while adding little overhead as the majority of compute lies in transformer layers before classification. The generator, on the other hand, does incur additional compute, and ELECTRA typically uses one with lower capacity than the discriminator (e.g. 12 layers and 768 hidden units). \cite{clark2020electra} also finds that this generally improves end task performance.

\hoifung{TODO: What's typical generator capacity in ELECTRA?}

\rob{Added information from electra paper along with citation}

% general, dom-spec, base, large
\subsection{Domain-Specific Pretraining}

The study of BERT pretraining originates in general domains such as newswire and web. For example, the original BERT model was pretrained on Wikipedia and Books \cite{devlin2018bert}. RoBERTa \cite{liu2019roberta}, another representative BERT model, was pretrained on a larger web text corpus. 
Biomedical text, however, is quite different from general-domain text, and domain-specific pretraining has been shown to substantially improve performance in biomedical NLP applications \cite{lee2020biobert,peng2019transfer,gu2021domainspecific}. In particular, \citet{gu2021domainspecific} conducted a thorough analysis on domain-specific pretraining, which highlights the utility of using a domain-specific vocabulary and pretraining on domain-specific text from scratch. 
We will build on their work and study how domain-specific pretraining might impact fine-tuning stability, especially for larger models.

%\hoifung{Don't we have results when fine-tuning by default is esp. troublesome for larger models?}
%\rob{See the bar chart (Figure 3) for the larger models study below}

\hoifung{update pubmedbert ref to ACM Special Issue}
\rob{done}
\hoifung{Ask Tristan for details, say To Appear}

% fine-tuning: MR, task-spec layer; variations in MR
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hoifung{
moving Fig/Tbl to top of column?

Fig 1: text and line look a bit faint; task-specific layer color didn't seem to match; "Freezing layer" -> "Freezing-layer"; "Removing layer" -> "Removing-layer"

Remove "Encoder layer" from legend: this suggests that other layers are not encoder, but they are. 

"Embedding layer" -> Embedding
"Task-specific layer" -> "Task-specific prediction"
}

\begin{figure}[!ht]
\centering
    \includegraphics[width=0.48\textwidth]{figs/stability_strategies.png}
    \caption{Strategies for increasing fine-tuning stability of a transformer-based model: freezing lower layers; decreasing learning rate for lower layers; reinitializing upper layers.
    }
    \label{fig:alternate_finetune_strategies_fig}
\end{figure}

\subsection{Meaning Representation}
Standard task-specific fine-tuning will take the top BERT layer as the meaning representation and pass it to the task-specific prediction component (e.g., a linear classification layer). 

review strategies - show graphs

It has been shown that BERT-based transformer models can be down-scaled whilst maintaining strong performance on NLP tasks \cite{sajjad2020poor}. Down-scaling these models has multiple advantages such as reducing fine-tuning times and memory usage. Figure~1\vphantom{\ref{fig:alternate_finetune_strategies_fig}} illustrates two strategies we apply to improve the efficiency of fine-tuning. Biomedical NLP practitioners often have to contend with computationally limited environments, particularly if a data set must be contained within a secure environment to mitigate privacy issues.

\hoifung{We could argue about down-scaling for efficiency; but think we should first highlight the more important bit of stability. 

What are the the best citations for stability? 

What about training longer and layer reinit? Cf. Fig 3.

Here we talked about removing. Did we try that in Fig 3?
}

\end{methods}

%\lipsum[2-4]


==> old/old-result-2.tex <==
\eat{
\begin{table}[ht]
\processtable{Comparison with different learning rate schedulers}
{\begin{tabular}{@{}llll@{}}
\midrule   &  constant & constant with warmup &  linear decay with warmup \\
\midrule
BC5-chem     &      92.79 &                 92.93 &                     \textbf{93.33} \\
BC5-disease  &      84.59 &                 84.94 &                     \textbf{85.62} \\
NCBI-disease &      87.64 &                 87.74 &                     \textbf{87.82} \\
BC2GM        &      83.54 &                 83.58 &                     \textbf{84.52} \\
JNLPBA       &      78.17 &                 78.44 &                     \textbf{79.10} \\
\midrule
EBM PICO     &      \textbf{74.01} &                 73.98 &                     73.38 \\
\midrule
ChemProt     &      75.92 &                 75.80 &                     \textbf{77.24} \\
DDI          &      80.19 &                 79.84 &                     \textbf{82.36} \\
GAD          &      79.25 &                 80.49 &                     \textbf{82.34} \\
\midrule
BIOSSES      &      91.52 &                 91.12 &                     \textbf{92.30} \\
\midrule
HoC          &      80.81 &                 79.70 &                     \textbf{82.32} \\
\midrule
PubMedQA     &      \textbf{57.98} &                 56.14 &                     55.84 \\
BioASQ       &      \textbf{88.07} &                 86.14 &                     87.56 \\
\midrule
BLURB score  &      80.53 &                 80.03 &                     \textbf{81.07} \\
\botrule
\end{tabular}}{}
\label{table:lr_scheduler}
\end{table}
}

\eat{
\begin{table}[!ht]
\processtable{The impact on BLURB score and BLURB tasks with scarce data when applying a layer-freezing finetuning strategy.} {\begin{tabular}{@{}ccccccc@{}}
\midrule
Frozen layers &  10 & 8 & 6 & 4 & 2 & 0 \\
\midrule
BC5-chem        & 91.05 & 91.95 & 92.69 & 93.17 & 93.30 & \textbf{93.33} \\  
BC5-disease     & 80.78 & 82.68 & 83.97 & 84.95 & 85.42 & \textbf{85.62} \\  
NCBI-disease    & 83.04 & 86.05 & 87.12 & 87.41 & \textbf{88.21} & 87.82 \\  
BC2GM           & 78.12 & 81.39 & 82.98 & 84.04 & \textbf{84.55} & 84.52 \\  
JNLPBA          & 76.26 & 78.24 & 78.68 & 79.00 & \textbf{79.16} & 79.10 \\
\midrule
EBM PICO        & 71.71 & 72.89 & 73.45 & \textbf{73.47} & 73.45 & 73.38 \\
\midrule
ChemProt        & 72.72 & 76.30 & 76.86 & \textbf{77.58} & 77.41 & 77.24 \\  
DDI             & 78.35 & 81.70 & 82.58 & 81.91 & \textbf{83.17} & 82.36 \\  
GAD             & 81.48 & 83.34 & 83.84 & \textbf{84.01} & 83.98 & 83.96 \\
\midrule
BIOSSES         & 92.36 & 93.74 & \textbf{93.90} & 93.45 & 92.93 & 92.30 \\
\midrule
HoC             & 82.26 & 82.84 & \textbf{83.02} & 82.73 & 82.52 & 82.32 \\
\midrule
PubMedQA        & 60.80 & \textbf{64.09} & 62.90 & 58.44 & 56.34 & 55.84 \\  
BioASQ          & 83.29 & 89.36 & \textbf{91.79} & 90.07 & 89.29 & 87.56 \\
\midrule
BLURB score     & 79.62 & 81.78 & \textbf{82.32} & 81.80 & 81.56 & 81.16 \\ 
\botrule
\label{table:freeze_vs_remove}
\end{tabular}}{}
\end{table}
}

\eat{
\begin{table}[!t]
\caption{Comparison of BLURB test performance using $\tt LARGE$ models (24 layers, 300M+ parameters).}
\resizebox{.4791\textwidth}{!}{
\begin{tabular}{@{}lllllll@{}}
    \hline
    & \multirow{2}{*}{\begin{tabular}{@{}l@{}}BERT\\-$\tt LARGE$\end{tabular} }
    & \multirow{2}{*}{\begin{tabular}{@{}l@{}}RoBERTa\\-$\tt LARGE$\end{tabular} }
    & \multirow{2}{*}{\begin{tabular}{@{}l@{}}BioBERT\\-$\tt LARGE$\end{tabular} }
    & \multirow{2}{*}{\begin{tabular}{@{}l@{}}BlueBERT\\-$\tt LARGE$\end{tabular}}
    & \multirow{2}{*}{\begin{tabular}{@{}l@{}}ELECTRA \\-$\tt LARGE$\end{tabular}}
    & \multirow{2}{*}{\begin{tabular}{@{}l@{}}PubMedBERT\\-$\tt LARGE$\end{tabular}} \\
    & & & & & \\
\midrule
BC5-chem         &       90.58 &          90.79 &          93.05 &           90.24 &          91.96 &             \textbf{93.23} \\
BC5-disease      &       82.35 &          82.38 &          84.97 &           82.93 &          84.57 &             \textbf{85.77} \\
NCBI-disease     &       86.10 &          87.27 &          \textbf{88.76} &           86.44 &          87.87 &             88.25 \\
BC2GM            &       82.30 &          82.24 &          84.21 &           80.86 &          83.41 &             \textbf{84.72} \\
JNLPBA           &       78.20 &          78.15 &          78.83 &           77.59 &          78.19 &             \textbf{79.44} \\
EBM PICO         &       72.82 &          \textbf{73.87} &          73.81 &           72.43 &          73.38 &             73.61 \\
ChemProt         &       73.88 &          75.89 &          77.79 &           71.31 &          75.41 &             \textbf{78.77} \\
DDI              &       80.05 &          81.52 &          81.53 &           78.99 &          81.43 &             \textbf{82.39} \\
GAD              &       78.31 &          73.97 &          81.01 &           73.86 &          81.50 &             \textbf{81.98} \\
BIOSSES          &       79.83 &          78.17 &          71.30 &           83.44 &          82.22 &             \textbf{90.29} \\
HoC              &       80.86 &          80.17 &          81.57 &           81.35 &          57.28 &             \textbf{82.57} \\
PubMedQA         &       50.76 &          54.24 &          54.68 &           49.28 &          55.20 &             \textbf{63.18} \\
BioASQ           &       75.36 &          81.03 &          78.93 &           70.43 &          79.93 &             \textbf{92.36} \\
\midrule
\begin{tabular}{@{}l@{}}BLURB\\score\end{tabular}
&       76.31 &          76.86 &          76.59 &           75.90 &          74.18 &             \textbf{81.93} \\
\midrule
\begin{tabular}{@{}l@{}}Delta\\over $\tt BASE$\end{tabular}
&        +0.35 &           +0.56 &          -3.67 &           -0.26 &          -1.84 &              +0.51 \\
\botrule
\end{tabular}}{}
\label{table:large}
\end{table}
}

\eat{
\begin{table}[!ht]
\caption{Evaluation of large models on BLURB}
\resizebox{.4725\textwidth}{!}{
\begin{tabular}{@{}lllllll@{}}
    \hline
    & \multirow{2}{*}{\begin{tabular}{@{}l@{}}BERT\\-Large\end{tabular}} & \multirow{2}{*}{\begin{tabular}{@{}l@{}}RoBERTa\\-Large\end{tabular} } & \multirow{2}{*}{\begin{tabular}{@{}l@{}}BioBERT\\-Large\end{tabular} } & \multirow{2}{*}{\begin{tabular}{@{}l@{}}BlueBERT\\-Large\end{tabular}} &
    \multicolumn{2}{c}{PubMedBERT}\\
    \cline{6-7}
    & & & & & Base & Large \\
\midrule
BC5-chem     &       90.58 &          90.79 &          93.05 &           90.24 &            \textbf{93.33} &             93.23 \\
BC5-disease  &       82.35 &          82.38 &          84.97 &           82.93 &            85.62 &             \textbf{85.77} \\
NCBI-disease &       86.10 &          87.27 &          \textbf{88.76} &           86.44 &            87.82 &             88.25 \\
BC2GM        &       82.30 &          82.24 &          84.21 &           80.86 &            84.52 &             \textbf{84.72} \\
JNLPBA       &       78.20 &          78.15 &          78.83 &           77.59 &            79.10 &             \textbf{79.44} \\
\midrule
EBM PICO     &       72.82 &          \textbf{73.87} &          73.81 &           72.43 &            73.38 &             73.61 \\
\midrule
ChemProt     &       73.88 &          75.89 &          77.79 &           71.31 &            77.24 &             \textbf{78.77} \\
DDI          &       80.05 &          81.52 &          81.53 &           78.99 &            82.36 &             \textbf{82.39} \\
GAD          &       78.31 &          73.97 &          81.01 &           73.86 &            \textbf{82.34} &             81.98 \\
\midrule
BIOSSES      &       85.90 &          87.77 &          91.84 &           84.12 &            \textbf{92.30} &             91.14 \\
\midrule
HoC          &       80.86 &          80.17 &          81.57 &           81.35 &            82.32 &             \textbf{82.57} \\
\midrule
PubMedQA     &       50.76 &          54.24 &          54.68 &           49.28 &            55.84 &             \textbf{63.18} \\
BioASQ       &       75.36 &          81.03 &          78.93 &           70.43 &            87.56 &             \textbf{92.36} \\
\midrule
\begin{tabular}{@{}l@{}}BLURB\\score\end{tabular}
&       77.33 &          78.46 &          80.02 &           76.01 &            81.07 &             \textbf{82.07} \\ \\
\botrule
\end{tabular}}{}
\label{table:large_models}
\end{table}
}

\eat{

From scratch improves over continual but best performance is achieved with domain specific vocabulary.
\begin{table}[!t]
\processtable{Continual pre-training from the pre-trained BERT model vs pre-training from scratch on domain specific text.} {\begin{tabular}{@{}llll@{}}
\toprule
    & \multirow{2}{*}{PubMed vocab}
    & \multicolumn{2}{c}{BERT vocab}\\
    \cline{3-4}
    & & continual & from scratch\\
\midrule
BC5-chem     &         \textbf{93.33} &                 93.31 &                    93.26 \\
BC5-disease  &         \textbf{85.62} &                 85.28 &                    85.43 \\
NCBI-disease &         87.82 &                 \textbf{88.53} &                    88.41 \\
BC2GM        &         \textbf{84.52} &                 83.93 &                    84.23 \\
JNLPBA       &         \textbf{79.10} &                 78.77 &                    78.91 \\
\midrule
EBM PICO     &         73.38 &                 73.52 &                    \textbf{73.75} \\
\midrule
ChemProt     &         \textbf{77.24} &                 76.70 &                    77.23 \\
DDI          &         82.36 &                 82.60 &                    \textbf{83.07} \\
GAD          &         \textbf{82.34} &                 80.30 &                    81.80 \\
\midrule
BIOSSES      &         92.30 &                 91.79 &                    \textbf{93.87} \\
\midrule
HoC          &         82.32 &                 81.74 &                    \textbf{83.01} \\
\midrule
PubMedQA     &         55.84 &                 55.92 &                    \textbf{57.15} \\
BioASQ       &         \textbf{87.56} &                 76.41 &                    79.00 \\
\midrule
BLURB score  &         \textbf{81.07} &                 79.84 &                    80.91 \\
\botrule
\end{tabular}}{}
\label{table:scratch_vs_continual}
\end{table}
}

\eat{
\begin{table}[!ht]
\processtable{The impact on BLURB score and BLURB tasks with scarce data when applying a layer-freezing finetuning strategy to PubMedBERT-Base and BioBERT-Base.} {\begin{tabular}{@{}ccccccc@{}}
\midrule
Frozen layers &  10 & 8 & 6 & 4 & 2 & 0 \\
\midrule
BIOSSES         & 92.36 & 93.74 & \textbf{93.90} & 93.45 & 92.93 & 92.30 \\
\midrule
PubMedQA        & 60.80 & \textbf{64.09} & 62.90 & 58.44 & 56.34 & 55.84 \\  
BioASQ          & 83.29 & 89.36 & \textbf{91.79} & 90.07 & 89.29 & 87.56 \\
\midrule
BLURB score     & 79.62 & 81.78 & \textbf{82.32} & 81.80 & 81.56 & 81.16 \\ 
\botrule
\midrule
Frozen layers &  10 & 8 & 6 & 4 & 2 & 0 \\
\midrule
BIOSSES & 86.52 & 88.47 & 88.72 & 88.87 & \textbf{89.71} & 89.52 \\
\midrule
PubMedQA & 59.80 & 63.66 & \textbf{64.24} & 63.10 & 62.28 & 60.24 \\
BioASQ & 77.79 & 84.71 & \textbf{85.86} & 85.64 & 85.71 & 84.14 \\
\midrule
BLURB score & 77.61 & 80.08 & \textbf{80.71} & 80.67 & 80.69 & 80.34 \\
\botrule
\label{table:freeze_vs_remove}
\end{tabular}}{}
\end{table}

\begin{figure}
\centering
    \includegraphics[width=0.48\textwidth]{figs/biosses_plot_3.png}
    \caption{Strategies to improve fine-tuning stability on the BIOSSES task for five large language models.
    }
    \label{fig:biosses_strategies}
\end{figure}}

\eat{

\begin{table}[!t]
\caption{Comparison of BLURB test performance using $\tt LARGE$ models (24 layers, 300M+ parameters).}
\resizebox{.4791\textwidth}{!}{
\begin{tabular}{@{}lllllll@{}}
    \hline
    & \multirow{2}{*}{\begin{tabular}{@{}l@{}}BERT\\-$\tt LARGE$\end{tabular} }
    & \multirow{2}{*}{\begin{tabular}{@{}l@{}}RoBERTa\\-$\tt LARGE$\end{tabular} }
    & \multirow{2}{*}{\begin{tabular}{@{}l@{}}BioBERT\\-$\tt LARGE$\end{tabular} }
    & \multirow{2}{*}{\begin{tabular}{@{}l@{}}PubMedELECTRA\\-$\tt LARGE$\end{tabular}}
    & \multirow{2}{*}{\begin{tabular}{@{}l@{}}ELECTRA \\-$\tt LARGE$\end{tabular}}
    & \multirow{2}{*}{\begin{tabular}{@{}l@{}}PubMedBERT\\-$\tt LARGE$\end{tabular}} \\
    & & & & & \\
\midrule
BC5-chem         &       90.58 &          90.79 &          93.05 &           90.24 &          91.96 &             \textbf{93.23} \\
BC5-disease      &       82.35 &          82.38 &          84.97 &           82.93 &          84.57 &             \textbf{85.77} \\
NCBI-disease     &       86.10 &          87.27 &          \textbf{88.76} &           86.44 &          87.87 &             88.25 \\
BC2GM            &       82.30 &          82.24 &          84.21 &           80.86 &          83.41 &             \textbf{84.72} \\
JNLPBA           &       78.20 &          78.15 &          78.83 &           77.59 &          78.19 &             \textbf{79.44} \\
EBM PICO         &       72.82 &          \textbf{73.87} &          73.81 &           72.43 &          73.38 &             73.61 \\
ChemProt         &       73.88 &          75.89 &          77.79 &           71.31 &          75.41 &             \textbf{78.77} \\
DDI              &       80.05 &          81.52 &          81.53 &           78.99 &          81.43 &             \textbf{82.39} \\
GAD              &       78.31 &          73.97 &          81.01 &           73.86 &          81.50 &             \textbf{81.98} \\
BIOSSES          &       79.83 &          78.17 &          71.30 &           83.44 &          82.22 &             \textbf{90.29} \\
HoC              &       80.86 &          80.17 &          81.57 &           81.35 &          57.28 &             \textbf{82.57} \\
PubMedQA         &       50.76 &          54.24 &          54.68 &           49.28 &          55.20 &             \textbf{63.18} \\
BioASQ           &       75.36 &          81.03 &          78.93 &           70.43 &          79.93 &             \textbf{92.36} \\
\midrule
\begin{tabular}{@{}l@{}}BLURB\\score\end{tabular}
&       76.31 &          76.86 &          76.59 &           75.90 &          74.18 &             \textbf{81.93} \\
\midrule
\begin{tabular}{@{}l@{}}Delta\\over $\tt BASE$\end{tabular}
&        +0.35 &           +0.56 &          -3.67 &           -0.26 &          -1.84 &              +0.51 \\
\botrule
\end{tabular}}{}
\label{table:large}
\end{table}

}

% Old table summary
\begin{table}[h]
\begin{tabular}{ |p{7.94cm}|  }
\hline
\textbf{Strategies to promote fine-tuning stability} \\
\hline
\label{table:finetune_stability_summary}
\begin{compactitem}
  \item \quad Fine-tune using ADAM with bias correction.
  \item \quad Significantly increase the number of training steps and lower learning rates.
  \item \quad Reinitializing the top encoder layers can provide a better overall initialization for the pre-trained model.
  \item \quad Freezing the lower encoder layers can promote fine-tuning stability whilst reducing training time significantly.
  \item \quad Following the standard procedure of finetuning ELECTRA, setting a layer-wise learning rate decay factor has a similar effect to freezing the lower encoder layers.
\end{compactitem}
\tabularnewline
\hline
\end{tabular}
\caption{Techniques used to reduce the variance in model performance on the small datasets that are part of BLURB and are prone to fine-tuning instability.}
\label{table:1}
\end{table}

==> old/old-result-3.tex <==
\section{Results}

% \hoifung{
% Fig 3: remove two BASE baseline lines, they end up distracting from appreciating variations; suggest to reorder as BERT, RoBERTa, Electra, BioBERT, PubMedBERT.
% }

%\hoifung{Clarify: Tbl1: single seq; }
%\rob{Single seq is models pretrained with a single sequence (segment ids are the same for all tokens regardless which sentence they are in}

% \hoifung{Assume our Electra is PubMed-from-scratch version, right? Let's add that to Tbl 1.}

% overview
In this section, we conduct a systematic study to evaluate the impact of various pretraining and fine-tuning aspects on task-specific performance.  
We ground our study on the Biomedical Language Understanding \& Reasoning Benchmark (BLURB)~\cite{gu2021domainspecific}. BLURB is a comprehensive benchmark for biomedical NLP, spanning thirteen datasets and six tasks: named entity recognition (NER), evidence-based medical information extraction (PICO), relation extraction, sentence similarity, document classification, and question answering. 
The BLURB score is the weighted average of test scores over the six tasks. To facilitate head-to-head comparison, we follow the train/dev/test setup from BLURB in all our experiments.

\subsection{Pretraining Objectives}

We first conduct ablation study to evaluate various components in the standard BERT pretraining objectives. Specifically, we experiment with skipping next-sentence prediction (NSP) during pretraining. Standard BERT pretraining inputs two text sequences (with two distinct segment IDs). We also experiment with inputting only a single sequence (with same segment ID). \autoref{table:pretraining} shows the results. In general, NSP has little impact on end task performance. However, pretraining with single sequences leads to substantial performance drop in the sentence similarity task (BIOSSES), presumably because this task requires comparison of two sentences and the training set is rather small, therefore pretraining with two text segments helps.

We also evaluate using the ELECTRA objectives. Surprisingly, it does not show any superiority over generative MLM pretraining as in standard BERT. In fact, for a number of tasks, such as sentence similarity, document classification, question answering, ELECTRA performs substantially worse. We note that these tasks also happen to have relatively small training sets. In the next subsection, we conduct a thorough analysis on fine-tuning optimization and show that in the more challenging biomedical NLP applications, ELECTRA fine-tuning can become rather unstable, which requires longer training time and additional adaptations such as reinitialization of top layers and freezing of bottom layers.

\hoifung{For ELECTRA, double check w. Hao on fine-tuning - did we use diff fine-tuning rate/schedule? Do we need to? Do we have results when those tasks perform better w. ELECTRA but require different fine-tuning?}

\begin{table}[!t]
\processtable{
Comparison of BLURB test performance using various pretraining objectives: standard BERT pretraining; BERT pretraining without NSP (i.e., MLM only); BERT pretraining with MLM only and single-sequence (single segment ID); ELECTRA.
} 
{
\begin{tabular}{@{}lccccc@{}}
\midrule
&  BERT & \begin{tabular}{@{}l@{}}BERT\\(no NSP)\end{tabular} & \begin{tabular}{@{}l@{}}BERT (no NSP,\\single seq)\end{tabular} & ELECTRA \\
\midrule 
BC5-chem     &     \textbf{93.33} &     93.21 &            93.20 &    93.00 \\
BC5-disease  &     \textbf{85.62} &     85.29 &            85.44 &    84.84 \\
NCBI-disease &     87.82 &     88.29 &            \textbf{88.68} &    87.17 \\
BC2GM        &     84.52 &     84.41 &            \textbf{84.63} &    84.03 \\
JNLPBA       &     \textbf{79.10} &     79.01 &            \textbf{79.10} &    78.57 \\
\midrule 
EBM PICO     &     73.38 &     \textbf{73.87} &            73.64 &    73.57 \\
\midrule 
ChemProt     &     \textbf{77.24} &     76.82 &            76.88 &    76.34 \\
DDI          &     82.36 &     \textbf{82.64} &            82.45 &    80.58 \\
GAD          &     \textbf{83.96} &     82.30 &            83.24 &    83.40 \\
\midrule 
BIOSSES      &     \textbf{93.46} &     93.12 &            75.50 &    80.24 \\
\midrule 
HoC          &     82.32 &     \textbf{82.37} &            81.91 &    81.28 \\
\midrule 
PubMedQA     &     55.84 &     56.40 &            \textbf{66.66} &    64.96 \\
BioASQ       &     87.56 &     83.57 &            85.64 &    \textbf{88.93} \\
\midrule 
\begin{tabular}{@{}l@{}}BLURB\\score\end{tabular}   &     \textbf{81.35} &     81.00 &            79.04 &    79.61 \\
\botrule
\end{tabular}
}{}
\label{tab:pretraining}
\end{table}
 

\begin{table}[!t]
\processtable{
Comparison of how different strategies to promote finetuning stability can boost transformer-based models, pretrained with different learning objectives, on Sentence Similarity (SS) and Question Answering (QA) tasks.
} 
{\begin{tabular}{l|cc|cc|cc|cc}
\toprule
\begin{tabular}{@{}l@{}}Pretraining\\objective\end{tabular} & \multicolumn{2}{c}{Baseline} & \multicolumn{2}{c}{\begin{tabular}{@{}l@{}}Layer-\\freeze\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}{@{}l@{}}Layer-wise\\decay\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}{@{}l@{}}Layer\\reinit\end{tabular}} \\
\midrule
&       SS &         QA &           SS &         QA &               SS &         QA &           SS &         QA \\
\midrule
BERT &    93.5 &       71.7 &        92.9 &      \textbf{76.3} &            93.4 &     74.3 &        \textbf{94.5} &      69.3 \\
BERT (no NSP) &    93.1 &     70.0 &        \textbf{94.0} &      \textbf{73.2} &            93.0 &     71.8 &        92.9 &      69.3 \\
\begin{tabular}{@{}l@{}}BERT (no NSP,\\single seq)\end{tabular} &     75.5 &      76.2 &        72.1 &      \textbf{78.0} &            74.1 &      77.5 &        \textbf{85.0} &     72.8 \\
& & & & & & & & \\
ELECTRA &    80.2 &     77.0 &        83.1 &      78.7 &            83.6 &      \textbf{79.1} &        \textbf{88.7} &      74.7 \\
\bottomrule
\end{tabular}}{}
\label{tab:base_stability}
\end{table}

\begin{table}[!t]
\processtable{
Comparison of how different strategies to promote finetuning stability can boost $\tt LARGE$ transformer-based model performance on Sentence Similarity (SS) and Question Answering (QA) tasks.
} 
{
\begin{tabular}{l|cc|cc|cc|cc}
\toprule
 & \multicolumn{2}{c}{Baseline} & \multicolumn{2}{c}{\begin{tabular}{@{}l@{}}Layer-\\freeze\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}{@{}l@{}}Layer-wise\\decay\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}{@{}l@{}}Layer\\reinit\end{tabular}} \\
\midrule
&       SS &         QA &           SS &         QA &               SS &         QA &           SS &         QA \\
\midrule
BioBERT-Large &     84.9 &       60.9 &         88.7 &       65.4 &             90.1 &       \textbf{67.0} &         \textbf{91.5} &       64.8 \\       
BlueBERT-Large &     82.4 &       59.9 &         84.6 &       62.7 &             84.8 &       \textbf{63.7} &         \textbf{86.2} &       63.0 \\       
\begin{tabular}{@{}l@{}}PubMedBERT\\-Large\end{tabular} &     91.1 &       77.8 &         91.2 &       79.3 &             90.9 &       \textbf{80.4} &         \textbf{91.3} &       76.9 \\
\begin{tabular}{@{}l@{}}PubMedELECTRA\\-Large\end{tabular} &     71.6 &       67.6 &         86.4 &       76.5 &             86.2 &       \textbf{79.1} &         \textbf{90.3} &       76.0 \\
\bottomrule
\end{tabular}
}{}
\label{tab:large_stability}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\eat{
We conduct experiments to evaluate the utility of the next sentence prediction task in BERT pre-training. We also use a single sequence as the pre-training input, as opposed to assigning different segment ids to multiple sequences that are conventionally fed into the model \cite{devlin2018bert}, to evaluate how this impacts the BLURB score. Since regular BERT is trained on sentence pairs, the two sentences have different segment ids to indicate which tokens belong to which sentence. We find that dropping NSP only decreases performance slightly. In addition pre-training with single sequence is only challenging on BIOSSES because of small number of training examples. Segment ids indicating different sentences is useful for this sentence similarity task, we speculate that it is challenging for the model to learn which tokens correspond to which sentence from just 64 training examples when the segment ids are identical for every token. We also find that the model pre-trained with a single sequence suffers from fine-tuning instability on BIOSSES and to get a reasonable score on this task, we must reinitialise the top layer of the encoder. We investigate strategies to promote fine-tuning stability, such as reinitializing the encoder layers, in Section 3.3.  
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Fine-Tuning Adaptations}

Table~3\vphantom{\ref{table:freeze_vs_remove}} highlights the datasets that are most responsible for the large gap in performance between the alternate fine-tuning strategies outlined in Figure~1\vphantom{\ref{fig:alternate_finetune_strategies_fig}}. The datasets BIOSSES, PubMedQA and BioASQ have the fewest number of training examples in BLURB and they are also require the most advanced language comprehension. When fine-tuning a model on these datasets freezing the lower encoder layers improves fine-tuning stability and drives the BLURB score higher. On the other hand removing encoder layers has a detrimental impact on model performance, possibly because such challenging tasks require more complex reasoning and higher-level features extracted in the upper encoder layers of a pre-trained model are useful for these tasks.

Figure~2\vphantom{\ref{fig:alternate_finetune_strategies_plot}} illustrates how the BLURB scores of PubMedBERT-Base and BioBERT-Base vary with the number of layers trained using these alternate fine-tuning strategies. As expected we see a drop in performance as we remove encoder layers consistent with \cite{sajjad2020poor}. However there is an unexpected gain in performance on BLURB when we freeze a fraction of the encoder layers. We investigate this phenomenon and Figure 3 illustrates how the layer freezing strategy improves fine-tuning stability on scarce data tasks. Since data in the biomedical is more expensive to label than in the general domain BLURB is particularly sensitive to performance on scarce data tasks.

Figure~3\vphantom{\ref{fig:biosses_strategies}} illustrates how effective some of the techniques summarised in Table~7\vphantom{\ref{table:finetune_stability_summary}} are at restoring fine-tuning stability to five large, pre-trained language models. We evaluate these techniques on the BIOSSES dataset since we find that the very small number of datapoints associated with this task make it particularly tricky to finetune large models on. It has been shown that setting the de-biasing terms in ADAM, training for longer and at lower learning rates and reinitializing the top layers of pre-trained models can significantly improve fine-tuning stability \cite{zhang2021revisiting} \cite{mosbach2021on}. We replicate these findings and find that the simple strategy of freezing lower encoder layers provides similar benefits, in particular for ELECTRA style models.

\hoifung{Electra: Is this PubMed-from-scratch or general-domain? Did we compare the two versions and verify that Pubmed one is better?}

For practitioners interested in fine-tuning large pre-trained biomedical language models we explore techniques to reduce the number of trainable layers in the model by comparing alternate strategies for fine-tuning. We also conduct an experiment to compare different learning rate schedulers for fine-tuning PubMedBERT-base on BLURB.
Hyper-parameter search is within the window 1e5 to 5e5 and 3 to 60 epochs. 

\subsection{Model Size}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[!t]
\processtable{
Comparison of BLURB test performance using $\tt LARGE$ models (24 layers, 300M+ parameters).
} 
{\begin{tabular}{lcccc}
\toprule
& \multirow{2}{*}{\begin{tabular}{@{}l@{}}BioBERT\\-$\tt LARGE$\end{tabular}} &  \multirow{2}{*}{\begin{tabular}{@{}l@{}}BlueBERT\\-$\tt LARGE$\end{tabular}} &  \multirow{2}{*}{\begin{tabular}{@{}l@{}}PubMedBERT\\-$\tt LARGE$\end{tabular}} &  \multirow{2}{*}{\begin{tabular}{@{}l@{}}PubMedELECTRA\\-$\tt LARGE$\end{tabular}} \\
& & & & \\
\midrule
BC5-chem     &          93.05 &           90.24 &             93.23 &                \textbf{93.25} \\
BC5-disease  &          84.97 &           82.93 &             \textbf{85.77} &                85.23 \\
NCBI-disease &          \textbf{88.76} &           86.44 &             88.25 &                88.19 \\
BC2GM        &          84.21 &           80.86 &             \textbf{84.72} &                84.47 \\
JNLPBA       &          78.83 &           77.59 &             \textbf{79.44} &                78.32 \\
\midrule
EBM PICO     &          73.81 &           72.43 &             73.61 &                \textbf{74.02} \\
\midrule
ChemProt     &          77.79 &           71.31 &             \textbf{78.77} &                77.26 \\
DDI          &          81.53 &           78.99 &             \textbf{82.39} &                80.37 \\
GAD          &          82.47 &           75.80 &             83.57 &                \textbf{83.93} \\
\midrule
BIOSSES      &          \textbf{91.53} &           86.18 &             91.31 &                90.33 \\
\midrule
HoC          &          81.57 &           81.35 &             \textbf{82.57} &                82.37 \\
\midrule
PubMedQA     &          56.30 &           55.18 &             \textbf{67.38} &                65.02 \\
BioASQ       &          78.93 &           72.21 &             \textbf{93.36} &                92.29 \\
\midrule
\begin{tabular}{@{}l@{}}BLURB\\score\end{tabular}  &          80.18 &           77.11 &             \textbf{82.62} &                81.96 \\
\midrule
\begin{tabular}{@{}l@{}} $\Delta$ $\tt BASE$\\model\end{tabular} &          -0.49 &            +0.15 &              +0.34 &                 \textbf{+0.45} \\
\bottomrule
\end{tabular}}{}
\label{tab:large_models_blurb}
\end{table}

\begin{table}[!t]
\processtable{
Comparison of which tasks in the BLURB benchmark suffer the greatest drops in performance when the upper layers of the transformer model are removed.
} 
{
\begin{tabular}{lcccc|c}
\toprule
 & \multicolumn{4}{c}{Layers removed } & Performance \\
& 0 & 2 & 4 & 6 & Drop \\
\midrule
BC5-chem        & 93.3 & 93.2 & 93.0 & 92.4 &  -0.93 \\
BC5-disease     & 85.6 & 85.4 & 85.2 & 84.3 &  -1.33 \\
NCBI-disease    & 87.8 & 88.4 & 88.0 & 87.4 &  -0.44 \\
BC2GM           & 84.5 & 84.3 & 83.5 & 82.1 &  -2.47 \\
JNLPBA          & 79.1 & 78.9 & 78.9 & 78.1 &  -1.03 \\
\midrule
EBM PICO        & 73.4 & 73.4 & 73.3 & 73.4 &  -0.05 \\
\midrule
ChemProt        & 77.2 & 76.1 & 73.4 & 72.7 &  \textbf{-4.50} \\
DDI             & 82.4 & 82.2 & 79.7 & 79.3 &  \textbf{-3.06} \\
GAD             & 84.0 & 82.3 & 80.2 & 79.2 &  \textbf{-4.75} \\
\midrule
BIOSSES         & 92.3 & 92.7 & 92.8 & 92.1 &  -0.18 \\
\midrule
HoC             & 82.3 & 82.5 & 82.4 & 82.0 &  -0.31 \\
\midrule
PubMedQA        & 55.8 & 51.2 & 49.8 & 50.1 &  \textbf{-6.08} \\
BioASQ          & 87.6 & 83.7 & 77.5 & 74.0 & \textbf{-13.56} \\
\bottomrule
\end{tabular}}{}
\label{tab:removed_layers}
\end{table}

In this subsection, we explore how model size impacts downstream fine-tuning performance. 
As mentioned in \autoref{sec:method}, BERT models come in two standard variations: $\tt BASE$ and $\tt LARGE$. Prior work such as \cite{gu2021domainspecific} often focuses on $\tt BASE$ models. We instead conduct a thorough analysis on $\tt LARGE$ versions. 

We first perform standard fine-tuning as in \cite{gu2021domainspecific} and compare the BLURB test performance using various $\tt LARGE$ models. \autoref{table:large} shows the results. As expected, for general-domain models (BERT and RoBERTa), $\tt LARGE$ generally improves over $\tt BASE$, although the latter performs relatively poorly to begin with. Surprisingly, for most biomed-specific models, using the $\tt LARGE$ model actually hurts test performance. The only exception is PubMedBERT \cite{gu2021domainspecific}, which uses domain-specific vocabulary and pretrains on biomedical text from scratch.

Upon close inspection, it appears that the degradation in performance for $\tt LARGE$ models primarily stems from fine-tuning instability, especially for tasks with small training sets, such as sentence similarity and question answering. 

\hoifung{TODO: move stabilized version here; should probably add another table w. sec 3.3 techniques to highlight the best PubMedBERT models!}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\eat{
We evaluate several large transformer models on BLURB and find that PubMedBERT-Large is the only large biomedical language model to outperform its corresponding base model, using the standard BERT finetuning procedure. In Section 3.3 we demonstrate how large models often suffer from fine-tuning instability and we identify techniques to minimise the effect of this on models that are challenging to fine-tune. When employing these techniques to stabilise model performance on the small and unstable BIOSSES dataset we can break the previous record for the best score on BLURB; for PubMedBERT pretrained on PubMed abstracts we can achieve a BLURB score of 82.09 and 82.35 for the corresponding model pretrained on PubMed abstracts and PMC fulltext. The greatest gains that large models have over base models typically come from tricky tasks that have scarce data such as question answering, indicating how large models can outperform base models in the few shot setting.
}


\subsection{Comparison with Off-the-Shelf Tools}

We explore PubMedBERT vs scispaCy on simple NER tasks and fidn that even on the simplest of tasks PubMedBERT offers superior performance. The lenient F1 score employed in Table 5 differs to the typical exact span matching used to evaluate NER tasks. The lenient F1 score allows for inexact matches at the entity boundaries, a correct prediction occurs when the model predicts the start and end of the entity span to be equal to the gold label span or contained within it.

\begin{table}[!t]
\processtable{Comparisons of PubMedBERT models vs scispaCy on NER tasks in the BLURB benchmark.} {\begin{tabular}{@{}lccc|cc@{}}
\toprule
& \multicolumn{3}{c}{scispaCy (md)} & \multicolumn{2}{c}{PubMedBERT}\\
& jnlpba & bc5cdr & max & $\tt BASE$ & $\tt LARGE$\\
\midrule
BC5-chem          & 7.70 &  91.42 &     91.42 & 95.18 &     \textbf{95.37} \\      
BC5-disease       &   2.09 &88.88 &     88.88 & 93.34 &     \textbf{93.74} \\      
NCBI-disease      &   12.94 &   74.64 &     74.64 & 95.22 &     \textbf{95.24} \\      
BC2GM             &  68.87 &      15.92 &     68.87 & 95.56 &     \textbf{96.05} \\  
JNLPBA            &   87.25 &     20.50 &     87.25 & 88.79 &     \textbf{88.81} \\
\midrule
\begin{tabular}{@{}l@{}}Avg. lenient\\ NER score\end{tabular} & 35.77 &    58.27 &     82.21 & 93.62 &     \textbf{93.84} \\
\botrule
\label{table:scispacy}
\end{tabular}}{}
\end{table}

\begin{table}[!t]
\processtable{Comparison of PubMedBERT and PubMedELECTRA models finetuned using the default setup vs extensive hyperparameter tuning combined with finetuning stability strategies. * indicates where train and dev data was combined for finetuning} {
\begin{tabular}{lcc|cc}
\toprule
& \multicolumn{2}{c}{PubMedBERT} & \multicolumn{2}{c}{PubMedELECTRA}\\
\toprule
\begin{tabular}{@{}l@{}}Finetuning\\procedure\end{tabular} & Default & Strategic & Default & Strategic\\
\midrule
BC5-chem     &       \textbf{93.33} &       93.30 &          93.19 &          93.32 \\
BC5-disease  &       \textbf{85.62} &       85.42 &          84.99 &          85.16 \\
NCBI-disease &       87.82 &       \textbf{88.21} &          87.68 &          87.73 \\
BC2GM        &       84.52 &       \textbf{84.55} &          83.79 &          83.79 \\
JNLPBA       &       79.10 &       \textbf{79.16} &          78.60 &          78.64 \\
\midrule
EBM PICO     &       73.38 &       73.45 &          73.70 &          \textbf{73.72} \\
\midrule
ChemProt     &       77.24 &       \textbf{77.41} &          76.54 &          76.74 \\
DDI          &       82.36 &       \textbf{83.17} &          80.58 &          81.09 \\
GAD          &       83.96 &       \textbf{84.01} &          83.40 &          83.98 \\
\midrule
BIOSSES      &       92.30 &       \textbf{94.49} &          80.24 &          92.01* \\
\midrule
HoC          &       82.32 &       \textbf{83.02} &          81.45 &          82.57 \\
\midrule
PubMedQA     &       55.84 &       63.92 &          \textbf{67.64} &          \textbf{67.64} \\
BioASQ       &       87.56 &       91.79 &          87.71 &          \textbf{92.07} \\
\midrule
\begin{tabular}{@{}l@{}}BLURB\\score\end{tabular}  &       81.16 &       \textbf{82.75} &          79.81 &          82.41 \\
\botrule
\end{tabular}}{}
\label{tab:large_models_blurb}
\end{table}


==> old/old-result.tex <==
\section{Results}

\hoifung{
Fig 3: remove two BASE baseline lines, they end up distracting from appreciating variations; suggest to reorder as BERT, RoBERTa, Electra, BioBERT, PubMedBERT.
}

%\hoifung{Clarify: Tbl1: single seq; }
%\rob{Single seq is models pretrained with a single sequence (segment ids are the same for all tokens regardless which sentence they are in}

\hoifung{Assume our Electra is PubMed-from-scratch version, right? Let's add that to Tbl 1.}

% overview
In this section, we conduct a systematic study to evaluate the impact of various pretraining and fine-tuning aspects on task-specific performance.  
We ground our study on the Biomedical Language Understanding \& Reasoning Benchmark (BLURB)~\cite{gu2021domainspecific}. BLURB is a comprehensive benchmark for biomedical NLP, spanning thirteen datasets and six tasks: named entity recognition (NER), evidence-based medical information extraction (PICO), relation extraction, sentence similarity, document classification, and question answering. 
The BLURB score is the weighted average of test scores over the six tasks. To facilitate head-to-head comparison, we follow the train/dev/test setup from BLURB in all our experiments.

\subsection{Fine-Tuning Adaptations}

Table~3\vphantom{\ref{table:freeze_vs_remove}} highlights the datasets that are most responsible for the large gap in performance between the alternate fine-tuning strategies outlined in Figure~1\vphantom{\ref{fig:alternate_finetune_strategies_fig}}. The datasets BIOSSES, PubMedQA and BioASQ have the fewest number of training examples in BLURB and they are also require the most advanced language comprehension. When fine-tuning a model on these datasets freezing the lower encoder layers improves fine-tuning stability and drives the BLURB score higher. On the other hand removing encoder layers has a detrimental impact on model performance, possibly because such challenging tasks require more complex reasoning and higher-level features extracted in the upper encoder layers of a pre-trained model are useful for these tasks.

\begin{table}[!ht]
\processtable{The impact on BLURB score and BLURB tasks with scarce data when applying the alternate fine-tuning strategies that involve freezing or removing encoder layers.} {\begin{tabular}{@{}llll@{}}
\midrule   &  Train all layers & First 6 layers frozen & Last 6 layers removed \\
\midrule
BIOSSES      &             92.30 &                  \textbf{93.90} &                   92.12 \\
\midrule
PubMedQA     &             55.84 &                  \textbf{62.90} &                   50.08 \\
BioASQ       &             87.56 &                  \textbf{91.79} &                   74.00 \\
\midrule
BLURB score  &             81.07 &                  \textbf{82.21} &                   78.42 \\
\botrule
\label{table:freeze_vs_remove}
\end{tabular}}{}
\end{table}

Figure~2\vphantom{\ref{fig:alternate_finetune_strategies_plot}} illustrates how the BLURB scores of PubMedBERT-Base and BioBERT-Base vary with the number of layers trained using these alternate fine-tuning strategies. As expected we see a drop in performance as we remove encoder layers consistent with \cite{sajjad2020poor}. However there is an unexpected gain in performance on BLURB when we freeze a fraction of the encoder layers. We investigate this phenomenon and Figure 3 illustrates how the layer freezing strategy improves fine-tuning stability on scarce data tasks. Since data in the biomedical is more expensive to label than in the general domain BLURB is particularly sensitive to performance on scarce data tasks.

\begin{figure}[!htb]
\centering
    \includegraphics[width=0.48\textwidth]{figs/blurb_frozen_dropped_layers_2.png}
    \caption{Comparing the alternate strategies for fine-tuning for both PubMedBERT-Base and BioBERT-Base. The BLURB score is evaluated for the two models for both freezing the lower encoder layers or removing the upper encoder layers.
    }
    \label{fig:alternate_finetune_strategies_plot}
\end{figure}

Figure~3\vphantom{\ref{fig:biosses_strategies}} illustrates how effective some of the techniques summarised in Table~7\vphantom{\ref{table:finetune_stability_summary}} are at restoring fine-tuning stability to five large, pre-trained language models. We evaluate these techniques on the BIOSSES dataset since we find that the very small number of datapoints associated with this task make it particularly tricky to finetune large models on. It has been shown that setting the de-biasing terms in ADAM, training for longer and at lower learning rates and re-initializing the top layers of pre-trained models can significantly improve fine-tuning stability \cite{zhang2021revisiting} \cite{mosbach2021on}. We replicate these findings and find that the simple strategy of freezing lower encoder layers provides similar benefits, in particular for ELECTRA style models.

\begin{figure}
\centering
    \includegraphics[width=0.48\textwidth]{figs/biosses_plot_3.png}
    \caption{Strategies to improve fine-tuning stability on the BIOSSES task for five large language models.
    }
    \label{fig:biosses_strategies}
\end{figure}

\begin{table}[ht]
\processtable{Comparison with different learning rate schedulers}
{\begin{tabular}{@{}llll@{}}
\midrule   &  constant & constant with warmup &  linear decay with warmup \\
\midrule
BC5-chem     &      92.79 &                 92.93 &                     \textbf{93.33} \\
BC5-disease  &      84.59 &                 84.94 &                     \textbf{85.62} \\
NCBI-disease &      87.64 &                 87.74 &                     \textbf{87.82} \\
BC2GM        &      83.54 &                 83.58 &                     \textbf{84.52} \\
JNLPBA       &      78.17 &                 78.44 &                     \textbf{79.10} \\
\midrule
EBM PICO     &      \textbf{74.01} &                 73.98 &                     73.38 \\
\midrule
ChemProt     &      75.92 &                 75.80 &                     \textbf{77.24} \\
DDI          &      80.19 &                 79.84 &                     \textbf{82.36} \\
GAD          &      79.25 &                 80.49 &                     \textbf{82.34} \\
\midrule
BIOSSES      &      91.52 &                 91.12 &                     \textbf{92.30} \\
\midrule
HoC          &      80.81 &                 79.70 &                     \textbf{82.32} \\
\midrule
PubMedQA     &      \textbf{57.98} &                 56.14 &                     55.84 \\
BioASQ       &      \textbf{88.07} &                 86.14 &                     87.56 \\
\midrule
BLURB score  &      80.53 &                 80.03 &                     \textbf{81.07} \\
\botrule
\end{tabular}}{}
\label{table:lr_scheduler}
\end{table}

For practitioners interested in fine-tuning large pre-trained biomedical language models we explore techniques to reduce the number of trainable layers in the model by comparing alternate strategies for fine-tuning. We also conduct an experiment to compare different learning rate schedulers for fine-tuning PubMedBERT-base on BLURB.
Hyper-parameter search is within the window 1e5 to 5e5 and 3 to 60 epochs. 

\begin{table}[!t]
\processtable{
Comparison of BLURB test performance using various pretraining objectives: standard BERT pretraining; BERT pretraining without NSP (i.e., MLM only); BERT pretraining with MLM only and single-sequence (single segment ID); ELECTRA.
%Simplified pre-training without the next sentence prediction task and using only a single input sequence where the segment ids are the same for all tokens in the input sequence.\label{Tab:01}
} 
{\begin{tabular}{@{}ccccc@{}}
\midrule   &  BERT &  BERT (no NSP) &  BERT (no NSP, single seq) TODO +ELECTRA \\
\midrule
BC5-chem     &     \textbf{93.33} &     93.21 &            93.20 \\
BC5-disease  &     \textbf{85.62} &     85.29 &            85.44 \\
NCBI-disease &     87.82 &     88.29 &            \textbf{88.68} \\
BC2GM        &     84.52 &     84.41 &            \textbf{84.63} \\
JNLPBA       &     \textbf{79.10} &     79.01 &            \textbf{79.10} \\
\midrule
EBM PICO     &     73.38 &     \textbf{73.87} &            73.64 \\
\midrule
ChemProt     &     \textbf{77.24} &     76.82 &            76.88 \\
DDI          &     82.36 &     \textbf{82.64} &            82.45 \\
GAD          &     \textbf{82.34} &     80.04 &            81.57 \\
\midrule
BIOSSES      &     92.30 &     \textbf{93.28} &            83.06 \\
\midrule
HoC          &     82.32 &     \textbf{82.37} &            81.91 \\
\midrule
PubMedQA     &     55.84 &     56.40 &            \textbf{66.66} \\
BioASQ       &     \textbf{87.56} &     83.57 &            85.64 \\
\midrule
BLURB score  &     \textbf{81.07} &     80.90 &            80.21 \\
\botrule
\end{tabular}}{}
\label{tab:pretraining}
\end{table}

\subsection{Pretraining Objectives}

We first conduct ablation study to evaluate various components in the standard BERT pretraining objectives. Specifically, we experiment with skipping next-sentence prediction (NSP) during pretraining. Standard BERT pretraining inputs two text sequences (with two distinct segment IDs). We also experiment with inputting only a single sequence (with same segment ID). \autoref{table:pretraining} shows the results. In general, NSP has little impact on end task performance. However, pretraining with single sequences leads to substantial performance drop in the sentence similarity task (BIOSSES), presumably because this task requires comparison of two sentences and the training set is rather small, therefore pretraining with two text segments helps.

We also evaluate using the ELECTRA objectives. Surprisingly, it does not show any superiority over generative MLM pretraining as in standard BERT. In fact, for a number of tasks, such as sentence similarity, document classification, question answering, ELECTRA performs substantially worse. We note that these tasks also happen to have relatively small training sets. In \autoref{sec:fine-tune}, we conduct a thorough analysis on fine-tuning optimization and show that in the more challenging biomedical NLP applications, ELECTRA fine-tuning can become rather unstable and requires longer training time and additional adaptations such as reinitialization of top layers and freezing of bottom layers.

\hoifung{Did we use reinit to attain 83.06 on BIOSSES? In general, should conduct h2h comparison by default.}

\hoifung{For ELECTRA, double check w. Hao on fine-tuning - did we use diff fine-tuning rate/schedule? Do we need to? Do we have results when those tasks perform better w. ELECTRA but require different fine-tuning?}

\hoifung{TODO: Add Electra PubMed pretraining and comparison w. general domain}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\eat{
We conduct experiments to evaluate the utility of the next sentence prediction task in BERT pre-training. We also use a single sequence as the pre-training input, as opposed to assigning different segment ids to multiple sequences that are conventionally fed into the model \cite{devlin2018bert}, to evaluate how this impacts the BLURB score. Since regular BERT is trained on sentence pairs, the two sentences have different segment ids to indicate which tokens belong to which sentence. We find that dropping NSP only decreases performance slightly. In addition pre-training with single sequence is only challenging on BIOSSES because of small number of training examples. Segment ids indicating different sentences is useful for this sentence similarity task, we speculate that it is challenging for the model to learn which tokens correspond to which sentence from just 64 training examples when the segment ids are identical for every token. We also find that the model pre-trained with a single sequence suffers from fine-tuning instability on BIOSSES and to get a reasonable score on this task, we must reinitialise the top layer of the encoder. We investigate strategies to promote fine-tuning stability, such as re-initializing the encoder layers, in Section 3.3.  
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\eat{

From scratch improves over continual but best performance is achieved with domain specific vocabulary.
\begin{table}[!t]
\processtable{Continual pre-training from the pre-trained BERT model vs pre-training from scratch on domain specific text.} {\begin{tabular}{@{}llll@{}}
\toprule
    & \multirow{2}{*}{PubMed vocab}
    & \multicolumn{2}{c}{BERT vocab}\\
    \cline{3-4}
    & & continual & from scratch\\
\midrule
BC5-chem     &         \textbf{93.33} &                 93.31 &                    93.26 \\
BC5-disease  &         \textbf{85.62} &                 85.28 &                    85.43 \\
NCBI-disease &         87.82 &                 \textbf{88.53} &                    88.41 \\
BC2GM        &         \textbf{84.52} &                 83.93 &                    84.23 \\
JNLPBA       &         \textbf{79.10} &                 78.77 &                    78.91 \\
\midrule
EBM PICO     &         73.38 &                 73.52 &                    \textbf{73.75} \\
\midrule
ChemProt     &         \textbf{77.24} &                 76.70 &                    77.23 \\
DDI          &         82.36 &                 82.60 &                    \textbf{83.07} \\
GAD          &         \textbf{82.34} &                 80.30 &                    81.80 \\
\midrule
BIOSSES      &         92.30 &                 91.79 &                    \textbf{93.87} \\
\midrule
HoC          &         82.32 &                 81.74 &                    \textbf{83.01} \\
\midrule
PubMedQA     &         55.84 &                 55.92 &                    \textbf{57.15} \\
BioASQ       &         \textbf{87.56} &                 76.41 &                    79.00 \\
\midrule
BLURB score  &         \textbf{81.07} &                 79.84 &                    80.91 \\
\botrule
\end{tabular}}{}
\label{table:scratch_vs_continual}
\end{table}
}

%\lipsum[7]

\subsection{Model Size}

%\lipsum[8-9]

% \multicolumn{2}{c}{\begin{tabular}{@{}l@{}}PubMedBERT\\base\end{tabular} }\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\eat{
\begin{table}[!ht]
\caption{Evaluation of large models on BLURB}
\resizebox{.4725\textwidth}{!}{
\begin{tabular}{@{}lllllll@{}}
    \hline
    & \multirow{2}{*}{\begin{tabular}{@{}l@{}}BERT\\-Large\end{tabular} } & \multirow{2}{*}{\begin{tabular}{@{}l@{}}RoBERTa\\-Large\end{tabular} } & \multirow{2}{*}{\begin{tabular}{@{}l@{}}BioBERT\\-Large\end{tabular} } & \multirow{2}{*}{\begin{tabular}{@{}l@{}}BlueBERT\\-Large\end{tabular}} &
    \multicolumn{2}{c}{PubMedBERT}\\
    \cline{6-7}
    & & & & & Base & Large \\
\midrule
BC5-chem     &       90.58 &          90.79 &          93.05 &           90.24 &            \textbf{93.33} &             93.23 \\
BC5-disease  &       82.35 &          82.38 &          84.97 &           82.93 &            85.62 &             \textbf{85.77} \\
NCBI-disease &       86.10 &          87.27 &          \textbf{88.76} &           86.44 &            87.82 &             88.25 \\
BC2GM        &       82.30 &          82.24 &          84.21 &           80.86 &            84.52 &             \textbf{84.72} \\
JNLPBA       &       78.20 &          78.15 &          78.83 &           77.59 &            79.10 &             \textbf{79.44} \\
\midrule
EBM PICO     &       72.82 &          \textbf{73.87} &          73.81 &           72.43 &            73.38 &             73.61 \\
\midrule
ChemProt     &       73.88 &          75.89 &          77.79 &           71.31 &            77.24 &             \textbf{78.77} \\
DDI          &       80.05 &          81.52 &          81.53 &           78.99 &            82.36 &             \textbf{82.39} \\
GAD          &       78.31 &          73.97 &          81.01 &           73.86 &            \textbf{82.34} &             81.98 \\
\midrule
BIOSSES      &       85.90 &          87.77 &          91.84 &           84.12 &            \textbf{92.30} &             91.14 \\
\midrule
HoC          &       80.86 &          80.17 &          81.57 &           81.35 &            82.32 &             \textbf{82.57} \\
\midrule
PubMedQA     &       50.76 &          54.24 &          54.68 &           49.28 &            55.84 &             \textbf{63.18} \\
BioASQ       &       75.36 &          81.03 &          78.93 &           70.43 &            87.56 &             \textbf{92.36} \\
\midrule
\begin{tabular}{@{}l@{}}BLURB\\score\end{tabular}
&       77.33 &          78.46 &          80.02 &           76.01 &            81.07 &             \textbf{82.07} \\ \\
\botrule
\end{tabular}}{}
\label{table:large_models}
\end{table}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[!t]
\caption{Comparison of BLURB test performance using $\tt LARGE$ models (24 layers, 300M+ parameters).}
\resizebox{.4791\textwidth}{!}{
\begin{tabular}{@{}lllllll@{}}
    \hline
    & \multirow{2}{*}{\begin{tabular}{@{}l@{}}BERT\\-$\tt LARGE$\end{tabular} }
    & \multirow{2}{*}{\begin{tabular}{@{}l@{}}RoBERTa\\-$\tt LARGE$\end{tabular} }
    & \multirow{2}{*}{\begin{tabular}{@{}l@{}}BioBERT\\-$\tt LARGE$\end{tabular} }
    & \multirow{2}{*}{\begin{tabular}{@{}l@{}}BlueBERT\\-$\tt LARGE$\end{tabular}}
    & \multirow{2}{*}{\begin{tabular}{@{}l@{}}ELECTRA \\-$\tt LARGE$\end{tabular}}
    & \multirow{2}{*}{\begin{tabular}{@{}l@{}}PubMedBERT\\-$\tt LARGE$\end{tabular}} \\
    & & & & & \\
\midrule
BC5-chem         &       90.58 &          90.79 &          93.05 &           90.24 &          91.96 &             \textbf{93.23} \\
BC5-disease      &       82.35 &          82.38 &          84.97 &           82.93 &          84.57 &             \textbf{85.77} \\
NCBI-disease     &       86.10 &          87.27 &          \textbf{88.76} &           86.44 &          87.87 &             88.25 \\
BC2GM            &       82.30 &          82.24 &          84.21 &           80.86 &          83.41 &             \textbf{84.72} \\
JNLPBA           &       78.20 &          78.15 &          78.83 &           77.59 &          78.19 &             \textbf{79.44} \\
EBM PICO         &       72.82 &          \textbf{73.87} &          73.81 &           72.43 &          73.38 &             73.61 \\
ChemProt         &       73.88 &          75.89 &          77.79 &           71.31 &          75.41 &             \textbf{78.77} \\
DDI              &       80.05 &          81.52 &          81.53 &           78.99 &          81.43 &             \textbf{82.39} \\
GAD              &       78.31 &          73.97 &          81.01 &           73.86 &          81.50 &             \textbf{81.98} \\
BIOSSES          &       79.83 &          78.17 &          71.30 &           83.44 &          82.22 &             \textbf{90.29} \\
HoC              &       80.86 &          80.17 &          81.57 &           81.35 &          57.28 &             \textbf{82.57} \\
PubMedQA         &       50.76 &          54.24 &          54.68 &           49.28 &          55.20 &             \textbf{63.18} \\
BioASQ           &       75.36 &          81.03 &          78.93 &           70.43 &          79.93 &             \textbf{92.36} \\
\midrule
\begin{tabular}{@{}l@{}}BLURB\\score\end{tabular}
&       76.31 &          76.86 &          76.59 &           75.90 &          74.18 &             \textbf{81.93} \\
\midrule
\begin{tabular}{@{}l@{}}Delta\\over $\tt BASE$\end{tabular}
&        +0.35 &           +0.56 &          -3.67 &           -0.26 &          -1.84 &              +0.51 \\
\botrule
\end{tabular}}{}
\label{table:large_models}
\end{table}

\hoifung{Electra: Is this PubMed-from-scratch or general-domain? Did we compare the two versions and verify that Pubmed one is better?}

In this subsection, we explore how model size impacts downstream fine-tuning performance. 
As mentioned in \autoref{sec:method}, BERT models come in two standard variations: $\tt BASE$ and $\tt LARGE$. Prior work such as \cite{gu2021domainspecific} often focuses on $\tt BASE$ models. We instead conduct a thorough analysis on $\tt LARGE$ versions. 

We first perform standard fine-tuning as in \cite{gu2021domainspecific} and compare the BLURB test performance using various $\tt LARGE$ models. \autoref{table:large_models} shows the results. As expected, for general-domain models (BERT and RoBERTa), $\tt LARGE$ generally improves over $\tt BASE$, although the latter performs relatively poorly to begin with. Surprisingly, for most biomed-specific models, using the $\tt LARGE$ model actually hurts test performance. The only exception is PubMedBERT \cite{gu2021domainspecific}, which uses domain-specific vocabulary and pretrains on biomedical text from scratch.

Upon close inspection, it appears that the degradation in performance for $\tt LARGE$ models primarily stems from fine-tuning instability, especially for tasks with small training sets, such as sentence similarity and question answering. 

\hoifung{TODO: We should add another table w. sec 3.3 techniques to highlight the best PubMedBERT models!}

\hoifung{TODO: Maybe we should reorder: first fine-tuning; then pretraining obj; then large.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\eat{
We evaluate several large transformer models on BLURB and find that PubMedBERT-Large is the only large biomedical language model to outperform its corresponding base model, using the standard BERT finetuning procedure. In Section 3.3 we demonstrate how large models often suffer from fine-tuning instability and we identify techniques to minimise the effect of this on models that are challenging to fine-tune. When employing these techniques to stabilise model performance on the small and unstable BIOSSES dataset we can break the previous record for the best score on BLURB; for PubMedBERT pretrained on PubMed abstracts we can achieve a BLURB score of 82.09 and 82.35 for the corresponding model pretrained on PubMed abstracts and PMC fulltext. The greatest gains that large models have over base models typically come from tricky tasks that have scarce data such as question answering, indicating how large models can outperform base models in the few shot setting.
}
  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% scispaCy
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Comparison with Off-the-Shelf Tools}

We explore PubMedBERT vs scispaCy on simple NER tasks and fidn that even on the simplest of tasks PubMedBERT offers superior performance. The lenient F1 score employed in Table 5 differs to the typical exact span matching used to evaluate NER tasks. The lenient F1 score allows for inexact matches at the entity boundaries, a correct prediction occurs when the model predicts the start and end of the entity span to be equal to the gold label span or contained within it.

\begin{table}[ht]
\processtable{scispaCy comparison} {\begin{tabular}{@{}lllll@{}}
\toprule
    & \multicolumn{3}{c}{scispaCy (en\_ner)} & \multirow{2}{*}{\begin{tabular}{@{}l@{}}PubMedBERT\\-base\end{tabular} }\\
    \cline{2-4}
     & jnlpba\_md & bc5cdr\_md & max &\\
\midrule
BC5-chem          & 7.70 &  91.42 &     91.42 &       \textbf{95.31} \\      
BC5-disease       &   2.09 &88.88 &     88.88 &       \textbf{93.29} \\      
NCBI-disease      &   12.94 &   74.64 &     74.64 &       \textbf{95.39} \\      
BC2GM             &  68.87 &      15.92 &     68.87 &       \textbf{95.72} \\  
JNLPBA            &   87.25 &     20.50 &     87.25 &       \textbf{88.90} \\
\midrule
\begin{tabular}{@{}l@{}}Avg. lenient\\ NER score\end{tabular} & 35.77 &    58.27 &     82.21 &       \textbf{93.72} \\
\botrule
\label{table:scispacy}
\end{tabular}}{}
\end{table}
